Extended Coopetitive Soft Gating Ensemble

This article is about an extension of a recent ensemble method called Coopetitive Soft Gating Ensemble (CSGE) and its application on power forecasting as well as motion primitive forecasting of cyclists. The CSGE has been used successfully in the field of wind power forecasting, outperforming common algorithms in this domain. The principal idea of the CSGE is to weight the models regarding their observed performance during training on different aspects. Several extensions are proposed to the original CSGE within this article, making the ensemble even more flexible and powerful. The extended CSGE (XCSGE as we term it), is used to predict the power generation on both wind- and solar farms. Moreover, the XCSGE is applied to forecast the movement state of cyclists in the context of driver assistance systems. Both domains have different requirements, are non-trivial problems, and are used to evaluate various facets of the novel XCSGE. The two problems differ fundamentally in the size of the data sets and the number of features. Power forecasting is based on weather forecasts that are subject to fluctuations in their features. In the movement primitive forecasting of cyclists, time delays contribute to the difficulty of the prediction. The XCSGE reaches an improvement of the prediction performance of up to 11% for wind power forecasting and 30% for solar power forecasting compared to the worst performing model. For the classification of movement primitives of cyclists, the XCSGE reaches an improvement of up to 28%. The evaluation includes a comparison with other state-of-the-art ensemble methods. We can verify that the XCSGE results are significantly better using the Nemenyi post-hoc test.

==> chapters/abstract__copy_.tex <==
\begin{abstract}
This article is about a recent \textit{ensemble method} called \textit{Coopetitive Soft Gating Ensemble (CSGE)} and the application on power forecasting as well as motion primitive forecasting of cyclists.
Several extensions are proposed to the original \textit{CSGE} within this article, making the \textit{ensemble} even more flexible and powerful.
The \textit{CSGE} has been used sucessfully in the field of wind power forecasting, outperforming common algorithms in this domain.
The major idea of the \textit{CSGE} is to weight the models regarding their observed performance during training on different aspects.
On the one hand, the \textit{CSGE} is used to predict the power generation on both wind- and solar farms. On the other hand, the \textit{CSGE} is applied to forecast the movement state of cyclists in the context of driver assistance systems.
Both domains have very different requirements and are non-trivial problems.
The two problems differ fundamentally in the size of the data sets and the number of features. In addition, power forecasting is based on weather forecasts that are subject to fluctuations in their features additionaly. In the movement primitive forecasting of cyclists, time delays contribute to the difficulty of the prediction.
The presented \textit{CSGE} reaches an improvement of the prediction performance of up to 11\% for wind power forecasting and 30\% for solar power forecasting compared to the worst model.
For the classification of movement primitives of cyclists the \textit{CSGE} reaches an improvement of up to 28\%.
The evaluation includes a comparison with other state-of-the-art \textit{ensemble methods}.
\end{abstract}


==> chapters/ausblick.tex <==
\section{Ausblick}
\label{sec:ausblick}

Dieser Abschnitt gibt einen Ausblick auf mögliche Erweiterungen Ihrer Arbeit. Erläuteren Sie auch an dieser Stelle, welche Schwierigkeiten sich bei der Bearbeitung ihres Themas ergaben. Was hätte man besser, anderst machen können? Was sollte zusätzlich noch gemacht / untersucht werden? Vielleicht konnten aus zeitlichen Gründen nicht mehr alle Ideen durchgeführt werden. 

==> chapters/einleitung__copy_.tex <==
\section{Introduction}
\label{sec:einleitung}

The main goal of machine learning (ML) is to create models from a set of training data, that have a high capability of generalisation.
Often the ML problems are so complex that one single model cannot handle the whole scope. A common approach is to have multiple prediction models, instead of using only one single model. The approach of combining multiple estimators is called \textit{ensemble method} or short \textit{ensemble}.
Figure \ref{ensemble_simple} shows a general ensemble architecture. Several predictors provide estimations for an input, which are then combined by an aggregation function.

\begin{figure}[H]
  \centering
    \includegraphics[scale=0.3]{images/basic_ensemble}
     \caption{Generic \textit{ensemble} architecture \label{ensemble_simple}}
\end{figure}

As aggregation function several strategies have been proposed in research as well in applications. The advantage compared to single models primarily relates to generalization performance and robustness \cite{ensemble_garcia}.
To formally summarize the generalization performance, the error of a machine learning model can be decomposed in two components, which is referred as \textit{bias-variance decomposition} \cite{bias_variance}:

\textbf{Bias} is a measurement of how closely the average estimation of the machine learning algorithm is able to approximate the target.

\textbf{Variance} is a measurement on how much the estimation of the machine learning algorithm fluctuates for varying training sets.

In \cite{hansen_salamon} and \cite{zhou}, it is shown that ensembles often lead to better results than using one single estimator, by minimizing both bias and variance and therefore result in strong models.\\
When considering the results of machine learning competitions like \textit{KDD}\footnote[1]{https://www.kdd.org/kdd-cup} or \textit{Kaggle}\footnote[2]{https://www.kaggle.com/competitions} over the last years, \textit{ensemble methods} often win the first places.
For all this reasons \textit{ensemble methods} are a promising approach to solve real world problems.\\
Despite their good generalization performance, well-known \textit{ensemble methods} such as \textit{Boosting} \cite{Schapire1990}, \textit{Bagging} \cite{Breiman1996} or \textit{Stacking} \cite{Smyth1999} have the disadvantage that the aggregation function is not human-readable. They can be considered as black box models.
This paper deals with a novel \textit{ensemble method} called \textit{CSGE}. 
The proposed \textit{ensemble method} attempts to circumvent this decisive disadvantage by forming the aggregation function according to different potentially influenceing aspects that are easy for humans to comprehend.
Besides an adaptation of this \textit{ensemble} approach, this work mainly focuses on the application and detailed evaluation of two very different use cases.



\subsection{Contribution}

The presented \textit{ensemble} algorithm is mentioned in \cite{gensler_sick_2017}, \cite{gensler_sick_probabilistic} and \cite{gensler_knn_approx} initially. However, the \textit{CSGE} is strongly designed and evaluated to the needs of wind power forecasting.
In this article, we present a \textbf{general approach} of the \textit{CSGE}, which allows the use for \textbf{regression} as well as \textbf{classification tasks}. In addition, we have extended the \textit{XCSGE} to forecast \textbf{multivariate predictions} and use arbitrary error scores.
Furthermore, we have generalized the concept of \textit{local weighting} and gained the possibility to use an \textbf{arbitrary machine learning method} for this purpose.\\
We investigate the performance of the extended \textit{CSGE} (\textit{XCSGE}) on \textbf{two use cases}, which include both regression and classification tasks. Both use cases have \textbf{very different requirements} and can be solved efficiently with \textit{ensemble} approaches. Besides the different size of the two data sets, the number of features differs strongly (30 or 65 features for wind- and solar power forecasting, respectively 738 features for classification of movement primitives). On the one hand, we use the implemented \textit{XCSGE} to predict the power generation of both wind- and solar farms. We model this problem as a regression problem. In addition, the weather models, which we use as the basis for our predictions, are subject to fluctuations which are taken into account by the \textit{XCSGE}.
On the other hand, we use the \textit{XCSGE} to predict the state of motion of a cyclist using smart devices. We model this task as a classification task. The main difficulty lies in the large number of physical features originating from the smart devices sensors (i.e. accelerometer and gyroscope).\\
In addition, we have evaluated the models that estimate the expected error for the \textit{local weighting}.

\subsection{Structure}
In the following, we give a short overview of the article by summarizing each chapter. Chapter \ref{sec:related_work} (Related Work) gives a short overview of common \textit{ensemble methods}. In addition, we consider \textit{ensemble methods} that are especially used in the fields of power generation and motion prediction.
In Chapter \ref{sec:method} (Methods), a brief overview of the necessary fundamentals of \textit{ensemble methods} and a detailed description of the \textit{XCSGE} is given.  In addition, the developed extensions, which are included in this article, are explained.
In Chapter \ref{energyforecast} (Renewable Energyforecast), we apply the \textit{XCSGE} to predict the power generation of wind- as well as solar farms. A detailed evaluation of the trained \textit{XCSGE} and a comparison with state-of-the-art \textit{ensemble methods} is given. We further investigate the performance of the \textit{local weighting} models.
In Chapter \ref{cyclists} (Cyclists Basic Movement Detection) we apply the \textit{XCSGE} to predict the motion primitives of cyclists using smart devices. A detailed evaluation of the trained models is given.
The article closes with Chapter \ref{sec:outlook} (Conclusion and Outlook). 






==> chapters/titlepage.tex <==
%
% Diplomarbeit mit LaTeX
% ===========================================================================
% This is part of the book "Diplomarbeit mit LaTeX".
% Copyright (c) 2002-2005,2007 Tobias Erbsland
% Copyright (c) 2005 Andreas Nitsch
% See the file diplomarbeit_mit_latex.tex for copying conditions.
%

\begin{titlepage}
    \begin{center}
    
		\begin{figure}
				\includegraphics[width=0.35\textwidth]{images/uni-logo}
				\hfill
				\includegraphics[width=0.35\textwidth]{images/ies-logo}
		\end{figure}

    \vspace*{0.5cm}

    \large{Department Electrical Engineering / Computer Science}\\
    \vspace*{0.5cm} \large{Department Intelligent Embedded Systems (IES)\\Prof. Dr. Bernhard Sick}

    \vspace*{2cm}
 		% BITTE EINES DER BEIDEN WÄHLEN!! %
    \large {PROJECT REPORT}\\
    \vspace*{1cm} \Huge {\textbf{Coopetitive Soft Gating Ensembles with interpretable weighting scheme for diverse applications} }\\
    \vspace*{1cm}

    \normalsize{submitted by} \\
    \large{Stephan Deist} \\
    \vspace*{1.5cm} \normalsize{\today}

    \vspace*{1cm}

        \begin{center}
            \begin{tabular}{ll}
             Advisor: Maarten Bieshaar and Jens Schreiber
            \end{tabular}
        \end{center}

    \end{center}
\end{titlepage}

